On Structuring Functional Programs with Monoidal Profunctors

We study monoidal profunctors as a tool to reason and structure pure functional programs both from a categorical perspective and as a Haskell implementation. From the categorical point of view we approach them as monoids in a certain monoidal category of profunctors. We study properties of this monoidal category and construct and implement the free monoidal profunctor. We study the relationship of the monoidal construction to optics, and introduce a promising generalization of the implementation which we illustrate by introducing effectful monoidal profunctors.

==> eptcsdata.tex <==
\providecommand{\firstpage}{134}
\providecommand{\publicationstatus}{Jeremy Gibbons and Max S. New (Eds.): Ninth Workshop on\\ Mathematically Structured Functional Programming (MSFP 2022)\\
EPTCS 360, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.360.7}{10.4204/EPTCS.360.7}}
\pdfoutput=1

